On the absence of pulses from pulsars

The aim of this thesis is to investigate the absence of pulses in pulsar, a phenomena also know as pulsar nulling. The motivation for the work done in thesis is listed in Chapter 2. A detailed discussion on the previous work carried out to investigate pulsar nulling phenomena is also included in Chapter 2. Chapter 3 discusses in details all the observations carried out for the thesis. In Chapter 4, details regarding the nulling behaviour of various pulsars are listed. Chapter 4 highlights the fact that nulling is unpredictable. Chapter 5 presents a comparison between two pulsars with high NFs. It is shown that both the pulsars exhibit similar bursting behaviour, but strikingly different quasi-periodicities and emission properties. Chapter 6 discusses the details regarding the simultaneous observations of two nulling pulsars at four different frequencies. These observations suggest that nulling is a frequency independent phenomena simultaneous occuring over a decade of frequency. Chapter 7 summaries the results obtained in three different studies along with their implications. The future work to extend the work carried out in the thesis is also listed in Chapter 7. The main conclusions of the thesis are as follow, (1) NF is not an ideal parameter to quantify nulling behaviour, confirmed firmly by comparing low NF pulsars as well as high NF pulsars, (2) Nulling occurs randomly with unpredictable length durations. Quasi-periodicities seen in the high NF pulsars can also be explained by the Markov models with a forcing function, (3) Nulling is an extreme form of mode-changing phenomena which occurs on a global magnetospheric scale, (4) Geometric reasons are less favoured as a likely cause of nulling phenomena due to the randomness and broadband behaviour reported in this thesis.

==> Introduction_arxiv.tex <==
/\chapter{Introduction}
% \graphicspath{{/home/vishal/My_paper/Thesis/Chapter1/}{/home/vishal/My_paper/Thesis/Chapter1/}{/home/vishal/My_paper/Thesis/Chapter1/}}
\graphicspath{{Images/}{Images/}{Images/}}

{\itshape Pulsating stars (aka Pulsars)} are one of the most exotic objects in the known  
Universe due to their unique nature. Pulsars are highly magnetised 
rotating neutron stars. They emit beams of radiation in a concentrated emission cone 
which sweeps the surrounding sky in a light-house manner. When this beam of radiation crosses 
the line-of-sight towards the observer, a pulse can be detected. 
This train of pulses has a unique period associated 
with it, which is the period of rotation of the pulsar. 
Pulsars are known to emit radiation from radio to gamma-rays 
frequency regime, although from widely spaced emitting regions 
with different emission mechanisms. However, this thesis particularly 
focuses on the study in the radio frequency regime only. 

\section{Pulsar Discovery}
The first pulsar was discovered serendipitously 
in the late 1960s \cite[]{hbp+68}. Jocelyn Bell, 
a graduate student from the Cambridge University, and her supervisor Anthony Hewish,  
were conducting experiments to study the interplanetary scintillations. 
During these investigations, a train of pulses was detected. 
In an interesting account by \cite{bell77}, the first ever recorded 
signal from a pulsar was noticed as ``a bit of \emph{scruff}" on a chart recorder. 
The observed train of pulses, with 1.33 second periodicity, were first thought to be 
terrestrial signal. However, regular appearance of this signal following the sidereal time, 
eliminated the possibility of terrestrial origin (the source was subsequently named  
CP 1919 which is now known as pulsar B1919+21).  
All different possibilities were considered, including a possible beacon from 
an extra-terrestrial intelligence civilization. However, after a few months of this   
discovery, couple of more such sources were found at different locations in the sky, 
making it clear that the recorded phenomena has a natural origin. 
The peculiar property of such short periodicity allowed \cite{hbp+68} 
to conclude that, compact objects such as white dwarfs and neutron stars 
could be the possible source. The suggestion that pulsars are rotating neutron 
stars was also provided by \cite{gold68}. This was indeed 
confirmed later when a pulsar with 33 millisecond periodicity was discovered 
powering the Crab nebula, which is a supernovae remnant \cite[]{pac68}. 

The existence of neutron star in a stellar life cycle 
was first predicted by \cite{bz34}. However, a possible 
detection of any signal from the neutron stars was never expected. 
Hence, the discovery of radio signals from pulsars became the single most 
significant event to prove the existence of neutron stars. 
Currently, more than 2000 pulsars are known which exhibit a plethora 
of observed phenomena. Pulsars are fantastic 
laboratory to test many physical and astrophysical problems. 
They were extensively used to study the interstellar medium.  
Pulsars are also proposed to be an important probe in the gravitational 
wave detection [see \cite{joshi13} for a review]. 
% 
% \section{Radio emission properties}
\section{Pulsar Toy model}
\label{pulsar_toy_sect}
Pulsar radio emission have been studied extensively to scrutinize 
the emission mechanism. The radio emission was found to be 
highly polarized. In an interesting study by \cite{rc69}, 
pulsar emission was shown to be originating near the magnetic 
field lines. The rotating vector model suggests, pulsar has a co-rotating 
radiation beam aligned with its magnetic axis. The angle between 
the rotation axis and the magnetic axis, also known as $\alpha$, 
produces pulsed radio emission (shown in Figure \ref{pulse_train}) 
every time the radiation beam sweeps the line-of-sight of the earth \cite[]{rc69}. 
This picture of the pulsar toy model is shown in Figure \ref{toy_model}. 

\begin{figure}[!h]
 \centering
 \includegraphics[width=1.2 in,height=5 in,angle=-90,bb=352 50 554 770]{Pulse_train_for_thesis.pdf}
 \caption[Pulse train from PSR B0809+74]{An observed train of pulses from PSR B0809+74 
 (here \emph{PSR} stands for Pulsating Source of Radio and the number 
 followed by it presents right-ascension and declination of the source)}
 % Pulse_train_for_thesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=352 50 554 770
 \label{pulse_train}
\end{figure}
% 
\begin{figure*}[!h]
 \begin{center}
   \centering
%    \hspace*{1.2in}
%   \includegraphics[bb=0 0 536 539]{pulsar_toy_gimp.jpg}
 % pulsar_toy_gimp.jpg: 536x539 pixel, 72dpi, 18.91x19.01 cm, bb=0 0 536 539
  \includegraphics[width=3 in,height=4 in,angle=0,bb=0 0 449 640]{pulsar_toy_gimp.jpg}
 % pulsar_toy_gimp.jpg: 449x540 pixel, 72dpi, 15.84x19.05 cm, bb=0 0 449 540
  \caption[Pulsar toy model]{The schematic diagram of a radio pulsar to illustrate various regions around the neutron star (not to scale). 
  The magnetic axis is misaligned with the rotation axis, which gives the peculiar pulsating properties to each pulsar.
  The field lines enclosing inside the light cylinder are classified the close field line region while 
  the field lines which cross the light cylinder belong to open field line region 
  (cartoon using the free 3D modeling package : {\itshape blender} \url{www.blender.org}).}
  \label{toy_model}
 \end{center}
\end{figure*}
 
The charged particles, bound to the magnetic field lines, are forced to corotate with the neutron star. 
However, as the distance from the neutron star rotation axis increases, the linear velocity of the rotation 
of the charge particles also increases up to speed of light. Beyond this boundary, 
the particles can not continue to corotate with the star. This boundary, also known 
as the \emph{light cylinder}, divides the pulsar magnetosphere in two different regions, 
namely the open field lines and the close field lines as 
illustrated in Figure \ref{toy_model}. The region of open field lines 
allows the charge particles to accelerate and escape the magnetosphere. The 
radio emission is generated inside this open field line regions. 
The details regarding the production of the radio emission is given in Section \ref{radio_emission_sect}. 

\section{Propagation of radio waves}
The radio waves generated by the pulsar pass through the Galactic interstellar medium (ISM)
before reaching the observer. During their travel, the signal experiences multiple 
propagation effects, such as dispersion, scattering and scintillation, discussed below. 
Some of these effects can be reverted to retrieve the original signal. 

\subsection{Pulse dispersion}
The ionised component of the interstellar medium disperses the passing signal by introducing a frequency dependent 
delay. Pulse at higher frequencies experiences relatively shorter delay compared to 
pulse at lower frequencies. The delay in pulse arrival times 
across a finite bandwidth can be seen in Figure \ref{dispersion}. 
% 
\begin{figure}[h]
 \centering
 \includegraphics[width=3 in,height=4 in,angle=-90,bb=50 50 554 770]{Dispersion_plot.pdf}
 % Dispersion_plot.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 554 770
 \caption[Pulse dispersion]{Pulse dispersion shown for a simulated pulsar, with period of around 1 sec and DM of 100 pc cm$^{-3}$. 
 The expected delay across the observed bandwidth of 100 MHz at 550 MHz is around half the pulsar period.}
 \label{dispersion}
\end{figure}
% 
Quantitatively, the delay, $\bigtriangleup{\tau}$ in arrival times between a high frequency, $f_{high}$, 
and a low frequency, $f_{low}$, can be given as \cite[]{handbook}, 
% 
\begin{equation}
 \bigtriangleup{\tau} ~ = ~ 4.15 ~ \times ~ \bigg[\bigg(\frac{f_{low}}{GHz}\bigg)^{-2}~ - ~\bigg(\frac{f_{high}}{GHz}\bigg)^{-2} \bigg] ~ 
 \times ~ \bigg(\frac{DM}{pc~cm^{-3} }\bigg)~ msec. 
\end{equation}
% 
Here the dispersion measure (DM), which is an integrated column density of electrons, 
can be calculated as, 
% 
\begin{equation}
 DM ~ = ~ \int_{0}^{d} {n_e} dl ~~ pc~{cm^{-3}}.  
\end{equation}
% 
Here, d is the distance to the pulsar and $n_e$ is the electron density of the ISM. For 
all the known pulsars, the DM can be measured very accurately by comparing the pulse delay 
between higher and lower frequency channels across the observed bandwidth (as seen in Figure \ref{dispersion}). 
The model of the electron density, known as NE2001, across various line-of-sights has been approximately 
measured from independent estimates \cite{NE2001}. Thus, DM of a pulsar also provides a good measure 
of its distance with $\sim$30\% uncertainty.  

The dispersion effects can easily be removed from the DM of the pulsar. 
The procedure to remove the dispersion smearing 
is known as the dedispersion. There are two different ways in which the dispersion 
can be reverted to retrieve the original signal (a) Incoherent dedispersion 
and (b) Coherent dedispersion. During the coherent dedispersion, a model 
of the ISM needs to be adapted to revert the phase delays. This procedure 
is generally carried out during the observation time itself. However, it is 
also possible to coherently dedisperse the recorded data as well. 
While, for the case of  incoherent dedispersion, signals are delay 
compensated for individual frequency channels.  

\subsection{Pulse scattering}
\label{pulse_scattering_sect}
Scattering of the pulsar signals manifest as an exponential tail 
at the trailing edge of the received pulse. The irregularities in the 
electron density of the ISM results in a one-sided broadening 
of the pulse. To scrutinize the scattering phenomena, the intermediate ISM can be presented 
as multiple patches with varying refractive index in a thin screen. 
These patches perturbs the phase of the impinging radio wave-front, causing 
a scatter of the resultant signal. A simplified screen approximation 
of the ISM is shown in Figure \ref{scattering_picture}, in which 
the multipath scattering can be seen at the observing end. Signals 
received by the observer from different patches arrive slightly  
later compared to signals that travelled unperturbed. Hence, an exponential 
tail can be observed once the leading phase of the pulse arrives. 

\begin{figure}[h!]
 \centering
%  \hspace*{-1.5in}
 \includegraphics[width=4.5 in,height=1.7 in,angle=0,bb=0 0 505 275]{Scattering_picture.jpeg}
 % Scattering_picture.jpeg: 673x366 pixel, 96dpi, 17.81x9.68 cm, bb=0 0 505 275
 \caption[Pulse scattering]{A simplified model of the ISM screen approximation. The pulsar signal undergoes 
 multipath scattering inside the ISM. The signals with different path lengths, refracted from 
 different ISM regions, arrive at the telescope with varying delay time-scales. This effect  
 causes the pulse to grow broader with an exponential tail at the trailing edge. [Figure adapted 
 from an original version in \cite{lor08}]}
 \label{scattering_picture}
\end{figure}
% 
As can be seen from Figure \ref{scattering_picture}, 
the signal to noise ratio (S/N) reduces substantially due 
to the scattering. If the scattering tail decay time-scales 
matches the pulsar period, pulse detection becomes a daunting task. 
The relation between the exponential decay time-scale, 
pulsar distance (d) and observing frequency (f) 
can be presented as \cite[]{handbook}, 
% 
\begin{equation}
 \tau_{s} ~ \propto ~ d^2 ~ f^{-4}. 
\end{equation}
% 
Lower frequencies show relatively longer tails due to the above given relation. 
Hence, most of the pulsar searches are conducted above 1 GHz. 
The ISM is also not uniform in different directions. The Galactic 
plan and specially the Galactic center are regions where the electron density highest 
and the line-of-sight passes through a longer path of electrons, 
making search for pulsars a more challenging task in these regions. 

\subsection{Pulse scintillation}
\label{scintillation_sect}
\begin{figure}[h!]
 \centering
 \includegraphics[width=3 in,height=5 in,angle=-90,bb=50 50 554 770]{ISS_plot_forThesis.pdf}
 % ISS_plot_forThesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 554 770
 \caption[The interstellar scintillation seen for the pulse peak intensities]
 {The interstellar scintillation seen for the pulse peak intensities. The top panel 
 shows the peak pulse intensity as a function of time. Note the gradual variations due to 
 the changing interference pattern from the turbulent ISM. The bottom panel shows peak pulse 
 energy after removal of the interstellar scintillation normalizing by the block averages.} 
 \label{ISS_plot}
\end{figure}

Closely similar to the scattering phenomena, single pulses from the pulsars 
undergo large pulse intensity fluctuations. This effect is similar to the 
optical twinkling of stars caused by the Earth's atmosphere. 
Figure \ref{pulse_train} shows varying pulse intensities,  
a combination of intrinsic and scintillation effects seen for all known 
pulsars. It was first reported by \cite{lr68}. 
The pulse scintillation is caused by the highly turbulent and inhomogeneous ISM \cite[]{sch68}. 
Different ISM patches, as mentioned in the Section \ref{pulse_scattering_sect}, 
also cause an interference pattern at the observer's plane. Due to the 
relative motion between the observer, the pulsar and the ISM patches, 
the interference pattern also moves across the observer's plane. 
The relative velocity shifts the enhanced and the reduced intensity 
regions to cause changes in the pulse intensity. The time-scale 
of this intensity fluctuation depends upon the aggregated relative 
velocity \cite[]{sch68}. Scintillation can 
also reduce the observed pulse intensity to go below 
the detection threshold, making the single pulse study a challenging task. 
\cite{sch68} has suggested that pulse scintillation are correlated only 
over a limited range of frequencies, also known as the \emph{scintillation 
bandwidth} ($\bigtriangleup{f}$) related to the observing frequency ($f$) as, 
$\bigtriangleup{f}{~\propto~}f^{4}$. This matched well with 
the early observations of ten pulsars by \cite{ric69}. 
The correlation bandwidth for different line-of-sights can be calculated using 
Galactic electron density model \cite[]{NE2001}. Hence, by using a relatively 
larger bandwidth than $\bigtriangleup{f}$, scintillation effects can be reduced.
 
Figure \ref{ISS_plot} shows only the peak pulse energy of around 5000 consecutive burst pulses, 
of PSR B0809+74 observed from the Giant Meterwave Radio Telescope (GMRT) 
at 325 MHz with 33 MHz bandwidth. The gradual fall and rise in the pulse 
intensity is clearly evident. For an unbiased treatment of the individual pulses,
pulse intensities can be averaged in consecutive blocks and each pulse can be 
normalized with their respective block average. 
The effective peak pulse intensities, normalized by their respective block average to 
remove the interplanetary scintillation effect, is also shown in Figure \ref{ISS_plot}.  

\section{Observed pulsar parameters} 
\subsection{Integrated profile} 
\begin{figure}[h!]
 \centering
 \includegraphics[width=5 in,height=3.2 in,angle=0,bb=0 0 350 252]{Profiles.pdf}
 % Profiles.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 410 302
 \caption[Integrated profiles]{Integrated profiles of six pulsars, observed from the GMRT 
 at 325 MHz. Note the differences in the shape and structure between various profiles.}
 \label{integrated_profile_example}
\end{figure}

Pulsar exhibits varying types of fluctuations in the shape of the 
individual pulses. However, after adding many hundreds or a few 
thousand pulses, a stable shape can be obtained which is known 
as the \emph{integrated profile} of the pulsar. 
The profile of a pulsar remains constant, at a given observing frequency, 
irrespective of the epoch of observations. The integrated profile is like a unique 
signature of the individual pulsar and it shows wide variety of shapes and structures across all known 
pulsars. A few such examples of integrated profiles, to highlight their different shapes, 
are shown in Figure \ref{integrated_profile_example}. The remarkable stability of the integrated 
profile suggest a stable emission process for each pulsar. Hence, the study 
of the integrated profiles is important to map the radio 
emitting regions. However, a few pulsars show switch between different 
integrated profiles, a phenomena known as \emph{mode-changing}, 
which tends to occur for a few hundred to a few thousand pulses (see Section \ref{mode-changing-sect} for details). 
There are also effects like geodetic precession which causes a gradual change 
in profile shapes, although number of pulsars, in which this effect is seen, are very few. 

\subsection{Period and slowdown}
The period of the pulsar, which corresponds to its rotation, is one of the 
pulsar parameter measured with high accuracy. The period does show a gradual slow down due 
to the loss in the rotational kinetic energy of the neutron star with time. 
However, this slowdown of the period is only one part in 10$^{15}$ second for 
normal pulsars. The slowdown of the pulsar, presented as $\pdot$ (= dP/dt), can be measured 
accurately to predict the period of the pulsar at each epoch of observations. 
As the gradual changes in the slowdown rate is related to the amount of energy release by the 
neutron star, young pulsars show higher slowdown rate compared to older pulsars. 
The rate of loss of rotation kinetic energy, the 
spin-down luminosity, can be presented as \cite[]{handbook}, 
% 
\begin{equation}
 \dot{E}~=~ -\frac{dE_{rot}}{dt} ~=~ -\frac{d(I\varOmega^2/2)}{dt} ~=~ -I\varOmega\dot{\varOmega} ~=~ \frac{4\pi^2I\dot{P}}{P^{3}}.  
\end{equation}
% 
Here, $I$ is the moment of inertia and $\varOmega~=~2\pi/P$ is the rotation angular frequency. 
For a normal pulsar with $P$ of 1 sec, $\pdot$ around 10$^{-15}$ s/s and $I$ of the order of $10^{45} ~ g ~ cm^2$ 
[assuming spherical shape with canonical values of mass around 1.4$M_{\odot}$\footnote{$M_{\odot}$ = 1 Solar Mass} 
and radius of 10 km \cite[]{handbook}], the loss of rotational energy is of the order of 10$^{31}$ ergs/sec. 
However, the radio luminosity of a pulsar is a significantly small fraction of this 
energy as most of the energy of the pulsar goes in the emission at X-rays and $\gamma$-rays frequencies 
along with the energy carried away by the particle winds and magnetic dipole emission. 

\begin{figure}[h!]
 \centering
 \includegraphics[width=3 in,height=4 in,angle=-90,bb=50 50 554 770]{All_PSR_data_p_pdot.pdf}
 % All_PSR_data_p_pdot.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 554 770
 \caption[$\ppdot$ diagram of around 2000 pulsars]{$\ppdot$ diagram of around 2000 pulsars. 
 Two cluster of points represent the normal and the millisecond pulsars population at their respective period range.
 A few points, extending from the normal pulsars population towards the upper right corner are the 
 neutron stars discovered at higher energies. [The data were obtained from the 
 \url{www.atnf.csiro.au/research/pulsar/psrcat} \cite[]{mhth05}]}
 \label{ppdot}
\end{figure}
% 
$P$ and $\pdot$ are unique parameters which can also be used to calculate other 
parameters such as the characteristic age and the magnetic field.  
Pulsar exhibits wide range of periods, starting from the fastest known pulsar 
PSR J1748$-$2446ad with period of around 1.3 msec \cite[]{hrs+06} to the slowest known pulsar 
PSR J2144$-$3933\footnote{Few high energy sources were found to show 
longer periods compared to this pulsar.} with period of around 8.5 sec \cite[]{mld+96}. 
Figure \ref{ppdot} shows the $P-\pdot$ diagram, obtained from around 2000 pulsars. 
The plot shows scatter of points with two loosely bound clusters with a bridge 
joining them. The clusters correspond to two main groups, 
which seem to show slightly different observational properties. 
Pulsars with period less than 30 msec belong to a special class 
known as the \emph{millisecond pulsars}. They correspond to old 
neutron stars which have been 'recycled' by phases of mass accretion 
from the binary companion, to radiate once again. The big cluster at relatively 
slow rotation rate, with periods between 0.1 to 1 sec, are the normal pulsars. 
In this thesis, radio emission properties of only the normal pulsars have been discussed. 

\subsection{Pulse Polarization}
\label{pulse_polrization_intro_sect}
As mentioned in Section \ref{pulsar_toy_sect}, pulsar signals are highly polarized. 
The plane of the linear polarization point towards the orientation of the 
magnetic field lines at the point of emission. Hence, pulse polarization measurements are useful to scrutinize 
the geometry of the radio emitting region. Using the radio observations, four Stokes 
parameters, I, Q, U and V can be obtained, where I is the total intensity of 
the signal, while V is the circular polarization intensity.  
The linear polarization intensity, obtained from Q and U profiles 
as L ($=\sqrt{Q^2+U^2}$), is also of great importance to investigate. 
Along with these parameters, it is also of interest to study the position angle (PA) of 
linear polarization (Equation \ref{PA_eq}) as a function of pulse phase. 
% 
\begin{equation}
PA~=~\frac{1}{2}{tan^{-1}\bigg(\frac{U}{Q}\bigg)} 
\label{PA_eq}
\end{equation}
The error in the PA can be measured as \cite[]{mli04},   
% 
\begin{equation}
 \bigtriangleup{PA}~=~\frac{\sqrt{(U\times\bigtriangleup{U})^2~+~(Q\times\bigtriangleup{Q})^2}}{2\times{L^2}}. 
\end{equation}
% 
Here, $\bigtriangleup{U}$ and $\bigtriangleup{Q}$ are the root mean square deviations  
from Stokes U and Q average profiles respectively. 

\cite{rc69} has demonstrated that the emission in the radio regime originates near the magnetic pole, 
using the PA changes across the pulse profile. 
In the proposed Rotating-vector model, 
\cite{rc69} demonstrated the expected shape of the PA angle changes as 
characteristic {\bf$S$}-shape curve by simple geometric arguments. 
The expected polarization angle swing, as the line-of-sight cross the magnetic field lines, 
matched perfectly well with the observed PA swing for many pulsars. 
It should be noted that a few pulsar also exhibit an abrupt 90$^\circ$ swing in the 
otherwise smooth {\bf$S$}-shape curve. These kind of changes tend to occur due to 
the presence of two different orthogonal polarization modes. The change in their dominance 
can cause such abrupt swing of 90$^\circ$. Figure \ref{rotating_vector_fig} shows an example 
of different polarization profiles obtained for 
PSR B0525+21\footnote[2]{www.jb.man.ac.uk/research/pulsar/Resources/epn}, 
along with the {\bf$S$}-shaped PA swing across the pulse profile. 
In principle, the observed PA swing can also help to derive 
other pulsar parameters, such as $\alpha$ and $\beta$ using the geometry. 
Here, $\beta$ (also known as the impact angle) is an angle between 
the magnetic pole and the center of the line-of-sight cut on the emission beam 
measured away from the rotation axis. However, a degeneracy can occur between 
an outer line-of-sight cut (positive $\beta$) and an inner line-of-sight 
cut (negative $\beta$) for limited range of active pulse longitude \cite[]{nv82}.  
% 
\begin{figure}[!h]
 \centering
 \subfigure[]{
 \centering
 \includegraphics[width=2.5 in,height=2.5 in,angle=0,bb=0 0 350 252]{B0525_PAswing_forThesis.pdf}
 % B0525_PAswing_forThesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 410 302
 \label{pa_swing}
 }
 \subfigure[]{
  \centering
 \includegraphics[width=2.5 in,height=1.8 in,angle=0,bb=0 0 281 242]{rotating_vector_los.jpg}
 % rotating_vector_los.jpg: 374x323 pixel, 96dpi, 9.90x8.55 cm, bb=0 0 281 242
 \label{rotatig_vector}
 }
 \caption[Polarization profile with the rotating vector model]{
 Polarization profiles with the rotating vector model.
 (a) The panel shows different polarization profiles for PSR B0525+21 observed 
 at 1.4 GHz [Archival data obtained from the EPN pulsar network\footnotemark[2]; 
 original observations by \cite{gl98}]. The total intensity is shown with red line 
 while the linear and circular polarization profiles are shown with 
 blue and green solid lines. The bottom panel shows the PA (magenta line) across the 
 pulse longitude with the measured error bars. The characteristic $S$-shaped 
 swing is clearly evident in the bottom panel. (b) The panel shows the top 
 view of the radiation beam, with magnetic field lines emanating around the 
 magnetic pole. The red line-of-sight cut is shown to trace the PA swing as 
 it passes through magnetic field lines of changing orientation, 
 highlighting the rotating vector model proposed by \cite{rc69}.}
 \label{rotating_vector_fig}
\end{figure}

As the pulsar signal passes through the interstellar medium, 
it also undergoes Faraday rotation, which is a frequency dependent 
rotation of the polarization angle. The effect can cause artificial changes 
in the PA, although these changes are large and can easily be distinguished 
from the intrinsic PA changes. However, a careful calibration 
is required using an artificial source before obtaining the four 
Stokes parameters. 

\section{Single pulse phenomena}
\subsection{Giant Pulses}
Pulsar in the Crab nebula was one of the first source discovered through 
its extremely strong burst pulses \cite[]{sr68}. These pulses, 
also known as the \emph{Giant pulses}, have peak intensities 
up to 1000 times higher than normal individual pulses. Detail study of 
these Giant pulses from the Crab pulsar has revealed that they 
are superposition of extremely narrow nanosecond duration structures \cite[]{hkw+03}. 
Currently, giant pulses are known to occur in around 10 pulsars. 
They are mostly reported in the millisecond pulsars \cite[]{kt00,rj01,J04}. 
They have also been reported in three regular pulsars 
\cite[]{ke04,EK05}, only at lower frequencies of 100 MHz, which remain to be verified 
at higher frequencies. In the earlier studies \cite[]{sr68,kt00,J04}, 
it was reported that giant pulses have significantly smaller 
pulse widths compared to average pulses. The expected brightness 
temperature of these pulses reached up to 10$^{37}$ K, making them  
the brightest source in the known Universe \cite[]{cbh+04}. 
They also tend to occur near the edge (either near the trailing edge or near the leading edge)
of the pulse profile. The emission mechanism behind the production 
of giant pulses, with this peculiar nature, still remain unidentified. 
% 
\subsection{Drifting}
\label{drifting_intro_sect}
\begin{figure}[h!]
 \centering
 \includegraphics[width=4 in,height=4 in,angle=0,bb=0 0 562 487]{Drifting_beam_combine.jpg}
 % Drifting_beam_combine.jpg: 749x649 pixel, 96dpi, 19.82x17.17 cm, bb=0 0 562 487
 \caption[Example of drifting subpulses in PSR B0809+74]{An example of drifting subpulses in PSR B0809+74. 
 (a) A stack of around 100 pulses are shown in the top panel
 with the average profile in the bottom panel, obtained from the GMRT observations at 325 MHz.
 Individual pulse intensities are shown with a color ramp from blue to red. Note the varying structure 
 of individual pulses with two (sometimes three) subpulses. The drifting towards the leading side 
 is clearly evident in the consecutive pulse sequence. (b) The rotating sub-beams carousal 
 with a line-of-sight cut is shown to demonstrate the drifting of subpulses each time the line-of-sight 
 cuts the radiation beam during each period. Two sets of sub-beams are shown (light blue and dark blue) to show 
 the displacement of sub-beams during a period interval.}
 \label{drifting_beam}
\end{figure}

A few pulsars tend to show individual pulses with multiple peaks (i.e. subpulses), 
although the integrated profiles are smooth with single component in many cases. 
For such pulsars, contiguous pulses are reported to show marching of these 
subpulses across the pulse longitude, also known as the \emph{drifting}. 
The drifting of the subpulses was first reported by \cite{dc68}. 
Figure \ref{drifting_beam}(a) shows sequence of observed pulses 
from PSR B0809+74. The drifting of the subpulses is clearly evident here 
with a periodicity of around 11 periods after which the pattern repeats itself 
(see Section \ref{rotating_carousal_sect} for more details regarding the drifting periodicities).
\cite{rs75} have suggested the cause of the periodicity due to a rotating 
carousal of sub-beams within a hollow radiation beam (as shown in Figure \ref{drifting_beam}(b)). 
Each time the line-of-sight passes across the radiation beam, it encounters 
a slightly different set of arrangements of the sub-beams because of their  
rotation around the magnetic pole. As these sub-beams are uniformly distributed, the 
patten repeats itself after certain number of periods as each sub-beam is replaced by an 
adjacent sub-beam. \cite{dr01} has proposed a method to determine the number of 
sub-beams in the rotating carousal. 

The periodicity of the drifting subpulses is defined as $P_3$ while 
the separation between the subpulses in the individual pulse 
is defined as $P_2$. A significant correlation was reported 
between the $P_3$ and pulsar age \cite[]{wol80,ran86}. 
However, in the largest survey conducted on the drifting pulsars 
\cite[]{wes06,wse07,wel07}, it was concluded that 
no such correlation exist. Drifting of subpulses can occur in both directions, 
from leading side to trailing side and vice-versa. 
\cite{ran86} has reported that pulsars do not have any preferred sense 
of drifting as equal number of pulsars were found exhibiting 
different drifting directions. \cite{wes06,wse07} has also concluded 
that drifting is an intrinsic property of emission mechanism. 
However, for a few pulsars it is not possible to detect classical 
drifting behaviour because their subpulses are disordered. 
As pulsar gets older, the sub-beams structure becomes more and more organized to 
produce detectable subpulse drifting pattern \cite[]{wes06,wse07}. 

\subsection{Mode-changes}
\label{mode-changing-sect}
\begin{figure}[!h]
 \begin{center}
 \subfigure[]{
 \centering
 \includegraphics[width=2 in,height=2.5 in,angle=-90,bb=50 50 554 770]{Both_mode_forThesis.pdf}
 % Both_mode_forThesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 554 770
 }
 \subfigure[]{
 \centering
 \includegraphics[width=2 in,height=2.5 in,angle=-90,bb=50 50 554 770]{Mode_profiles_forThesis.pdf}
 % Mode_profiles_forThesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=50 50 554 770
 }
 \caption[Two examples of mode-changing pulsars]{Two examples of mode-changing pulsars PSRs (a) J1725$-$4043 (b) B2319+60, 
 observed from the GMRT at 325 MHz. Note the clear differences in the profiles for different modes.}
 \label{mode-changing-fig}
 \end{center}
\end{figure}

The integrated profile of a pulsar is known to be one of the stable parameter 
and in most cases, characterising cuts across the radiation beam.
However, a few pulsars display switching between different integrated profiles. 
This phenomena is known as the \emph{mode-changing}. In all mode-changing pulsars, 
one of the profile mode is more favoured over the other. This can be distinguished 
by measuring the amount of time pulsar spends during each profile mode. 

Figure \ref{mode-changing-fig} shows two examples of mode-changing pulsars. 
PSR J1725$-$4043 shows two different modes with different intensities in the 
trailing component. However, PSR B2319+60 shows three different modes 
with significantly different profiles \cite[]{wf81}. The transition between 
different modes are rather sudden for both these pulsars. 
In many pulsars, the modes are classified as the normal mode/s 
(for more frequent modes) and abnormal mode/s (for non-frequent modes). 
Mode-changes also manifests itself in the form of changing drift rates with 
different modes (see Section \ref{null_dritft_corr_sect}). 
For example, PSR B2319+60 shows slightly different drifting periodicities between  
Mode-A to Mode-B, while the Mode-C shows disordered subpulses \cite[]{wf81}. 

\cite{ran86} has tabulated different mode-changing pulsars and concluded that 
mode-changing is mostly observed in pulsars with multiple component profiles. 
The intensity of the central component was reported to enhance 
during the abnormal modes \cite[]{ran86}. A few pulsars also show 
significant changes in different polarization profiles, along with 
the total intensity profiles, indicating a global magnetospheric change. 
Recently, \cite{wmj07} has enhanced the number of known nulling 
pulsars by identifying mode-changing phenomena in around 6 pulsars. 
 
\subsection{Pulse Nulling}
\begin{figure}[h!]
 \centering
 \includegraphics[width=1.5 in,height=5 in,angle=-90,bb=352 50 554 770]{Pulse_train_forThesis.pdf}
 % Pulse_train_forThesis.eps: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=352 50 554 770
 \label{nulling_example}
 \caption[Nulling in single pulses]{A sequence of pulses from PSR B2319+60 observed at 1420 MHz 
 from the Westerbork Synthesis Radio Telescope. The nulling in pulses is clearly evident.}
\end{figure}

The abrupt cessation of pulsed radio emission for 
several pulse periods, exhibited by many pulsars, 
has remained unexplained despite the discovery 
of this phenomenon in many radio pulsars. 
This phenomenon, called \emph{pulse nulling}, was first 
discovered in four pulsars in 1970 \cite[]{bac70}. 
Subsequent studies have revealed pulse nulling 
in about 100 pulsars to date \cite[]{bac70, rit76, big92a, viv95, wmj07}. 

The fraction of pulses with no detectable 
emission is known as the nulling fraction (NF) 
and is a measure of the degree of nulling in 
a pulsar. However, NF does not specify 
the duration of individual nulls, nor does it 
specify how the nulls are spaced in time. 
Nulling can also considered to be an extreme form of mode-changing 
phenomena \cite[]{wmj07}, in which pulsar emission 
goes below the detection threshold. Chapter 2 discusses 
the nulling phenomena in full detail. 

\section{Outline of the thesis}
The aim of this thesis is to investigate the absence of pulses 
in pulsar, a phenomena also know as pulsar nulling. 
The outline of the thesis is as follows. 
The motivation for the work done in thesis 
is listed in Chapter 2. It also discusses the 
emission mechanism as proposed by the standard model. 
A summary on the previous work carried out to investigate the 
pulsar nulling phenomena is also included in Chapter 2. 
Chapter 3 discusses in details all the observations 
carried out for the work that has been reported in thesis. 
Observations from various radio telescopes are discussed 
and compared in the similar chapter. The common analysis techniques deployed 
during most of the observations are also listed 
in Chapter 3. In Chapter 4, details regarding the 
nulling behaviour of various pulsars are listed. 
The comparison has been made between similar NF pulsars 
in order to demonstrate that, the NF does not quantify nulling 
behaviour in full details. Chapter 4 also highlights the fact 
that nulling is unpredictable. Chapter 5 presents a 
comparison between two pulsars with high NFs. It is shown 
that both the pulsars exhibit similar bursting behaviour, 
but strikingly different quasi-periodicities and emission properties. 
Chapter 6 discusses the details regarding the simultaneous observations 
of two nulling pulsars at four different frequencies. 
Chapter 7 summaries the results obtained in three different studies 
along with their implications. The future work to extend the work carried 
out in the thesis is also listed in Chapter 7.  

% \newpage
% 
% \bibliographystyle{mn2e.bst}
% \bibliography{psrrefs.bib,modpsrrefs.bib,mybib.bib,modrefs.bib}
% \end{document}

==> synopsis_arxiv.tex <==
\chapter{Synopsis} 
\noindent\rule{16cm}{1pt} \\
{\bf\large Thesis title : On the absence of pulses from pulsars  \\
 Vishal Gajjar \\
 Supervisor : Dr. Bhal Chandra Joshi \\}
\noindent\rule{16cm}{1pt}

Pulsars are one of the most fascinating objects in the known Universe. The very nature of 
their regular pulsation led to their discovery in the early days. They  
were the first to provide sound evidence about the existence of the neutron stars. 
In the last 47 years since the discovery of these objects, extensive 
research has been carried out to investigate the origin of the pulsar radiation. 
There have been many attempts to scrutinize the bright radio emission seen from 
pulsars by utilizing numerous observed phenomena. One of such phenomena is 
the rapid shape-changes in the observed single pulses in spite of their average 
profile showing remarkable stability for observations separated by decades. 
The sporadic nature of the single pulses provides important clues regarding the chaotic 
nature of the pulsar radiation. Thus, enormous amount of research 
have been focused on the modelling of the single pulses. 
There are different types of single pulse phenomena seen in 
the radio pulsar \emph{viz.}  drifting, nulling and mode-changing, 
which also shows interdependence in certain cases. Drifting 
and mode-changing has been modelled to some extent by many 
previous studies. However, nulling is one of the  
unexplained phenomena seen in the radio pulsars. 
The absence of emission in the individual single pulses 
has defied satisfactory explanation since its discovery 
44 years ago. 

Nulling in the radio pulsars has been reported by \cite{bac70} 
for the first time in four pulsars. Since its discovery, around 109 
pulsars were reported to show prominent nulling behaviour in their 
single pulses. Nulling in pulsars has been historically quantified 
as the fraction of observed null pulses, also known as the \emph{nulling fraction} (NF). 
In order to find the operating mechanism that causes only a few pulsars 
to exhibit noticeable nulling behaviour, NFs were 
compared with many pulsar parameters by various groups 
\cite[]{rit76,ran86,big92a,viv95,wmj07}.
However, no strong correlation between the NF and any pulsar parameter 
has been reported to date. \cite{rit76} has reported that if the pulsar
period is long, it is likely to have high nulling fraction compared to short
period pulsars. As the period of the pulsar is directly related to its 
characteristic age, \cite{rit76} speculated that pulsars 
die with increasing fraction of nulls in them. 
Contrary to that, \cite{ran86} presented an alternative hypothesis 
of correlation with the profile classes, where no dependence 
was noticed between NF and age of the pulsar in a similar profile
morphological class. It was extensively shown 
in a study of around 60 pulsars, that the nulling fraction is likely
to be less than 1\% in pulsars exhibiting core component, while, it is more
likely to have higher nulling fraction in pulsars exhibiting conal profile \cite[]{ran86}. 
In a separate study by \cite{big92a}, NF was confirmed to show correlation 
with the profile classes along with a few weak correlations. However, 
\cite{wmj07} has shown that nulling does not show correlation with 
profile morphological classes as profiles with almost all classes 
show similar nulling behaviour. Moreover, \cite{wmj07} suggested that nulling 
is an extreme form of mode-changing phenomenon. 
Thus, there is no common agreement between different 
studies regarding the true nature of any correlation. 

The degree and form of pulse nulling varies from 
one pulsar to another. On one hand, there are 
pulsars such as PSR B0826$-$34 \cite[]{dll+79}
which null most of the time, and PSR J1752+2359 
\cite[]{lwf+04}, which exhibits no radio emission for 
3 to 4 minutes. In contrast, pulsars such as PSR B0809+74 
show a small degree of nulling \cite[]{la83}. 
Pulse nulling is frequent in pulsars such as PSR B1112+50, while it is very 
sporadic in PSR B1642$-$03 \cite[]{rit76}. 
Moreover, the pulsed emission abruptly 
declines by more than two orders of 
magnitudes during these nulls \cite[]{la83,vj97}, 
which are as yet not well understood. While 
nulling pulsars have been known for last three 
decades, the recently discovered new class of sources, 
such as Rotating Radio transients 
\cite[]{mll+06,km11,bjb+12} and 
intermittent pulsars \cite[]{klo+06,crc+12,llm+12}, 
also show a behaviour similar to classical nullers 
and are increasingly believed to be nulling 
pulsars \cite[]{bjb+12}, indicating that 
nulling occurs in a significant fraction of pulsar population.

Pulsar emission at different radio frequencies, 
originates at different locations in the pulsar magnetosphere \cite[]{kom70}. 
There are very few long simultaneous 
observations of nulling pulsars reported so far 
in the literature. In a simultaneous single pulse study 
of two pulsars, PSRs B0329+54 and B1133+16 at 327 and 2695 MHz, 
\cite{bs78} showed highly correlated pulse energy 
fluctuations. Simultaneous observations of 
PSR B0809+74 for about 350 pulses 
indicated that only 6 out of 9 nulls were simultaneous 
at 102 and 408 MHz \citep{dls+84}. About half of nulls 
were reported to occur simultaneously at 325, 610, 1400 
and 4850 MHz for PSR B1133+16 \citep{bgk+07}. In contrast, 
simultaneous nulls were reported at 303 and 610 MHz for 
PSR B0826$-$34 \citep{bgg08}. 
It is not clear if nulling represents a global 
failure of pulse radiation or is due to a shift in pulsar 
beam manifesting as lack of emission at the 
given observation frequency due to the geometry 
of pulse emission. 

In light of all these previous investigations, 
long, sensitive, and preferably simultaneous 
observations at multiple frequencies 
of a carefully selected sample of pulsars are 
motivated. Thus, the aim of this thesis is to quantify, model  
and compare nulling behaviour between different classes of pulsars  
to scrutinize the true nature of the nulling phenomenon. 

In this thesis, main results on three main investigations 
are discussed with the necessary background for each of them. 
In Chapter 1, basic introduction 
to the pulsars is provided. Details regarding the 
structure of the pulsar surroundings and origin of 
the radio emission are briefly derived in Chapter 2. 
Observations conducted for each investigation, are 
summarised with necessary details in Chapter 3. 
Further three chapters discuss results on 
the individual study. Chapter 4 presents results 
on the survey of nulling pulsar conducted using the GMRT. 
A comparison study between two high nulling fraction pulsars 
are discussed in Chapter 5. Unique simultaneous multi-frequency 
observations of two pulsars are summarised in Chapter 6. 
Chapter 7 presents summary of all the obtained results 
in the thesis along with a comprehensive view 
about the nulling behaviour suggested by our observations. 

The chapter wise summary of this thesis is given below. 
First three chapters provide necessary background, 
along with the details regarding various observations. 

\section*{\underline{\underline{Introduction}}}
Introduction to pulsars, including their discovery and peculiar 
observed properties, are discussed in \emph{Chapter 1}. 
A simple pulsar toy model is presented to explain the 
pulsating nature of this source. Radio waves 
from the pulsar, travelling through the interstellar medium, 
undergo numerous propagation related effects. A few of these effects 
can reduce the pulse energy to zero level. These effects 
could imitate intrinsic phenomenon like pulsar nulling. 
Thus, they are briefly explained to highlight their true nature. 
Different observed pulsar parameters and their stability 
on various time-scales are also discussed in the chapter. 
Various single pulse phenomena reported in the thesis are 
briefly introduced with examples. 

\emph{Chapter 2} aims to provide necessary background 
about the currently known radio emission mechanism physics of the pulsars. 
It starts with a discussion on the structure of the neutron star along with the 
properties and composition of its surface, which were used to 
build the standard pulsar emission model proposed by \cite{rs75}. 
Origin of the coherent radio emission due to the growth in the 
two stream instability is briefly reviewed. This chapter 
also summarises, in detail, all previous studies conducted to investigate 
pulsar nulling phenomena. Different models proposed over the 
years to explain the mode-changing phenomenon are also listed  
in this chapter to relate them to pulse nulling in extreme 
conditions. Towards the end, primary incentives for the 
work reported in this thesis are listed in order 
to assess these models. 

Details regarding all observations, reported in this 
thesis, are discussed with full details in \emph{Chapter 3}. 
Justification regarding the selections of sources 
and observing frequencies for different objectives are 
elaborated in this chapter. 
In this thesis, observations from 
four different telescopes has been reported \emph{viz.} 
the GMRT, the WSRT, the Arecibo telescope and the Effelsberg 
radio telescope. Details about all these telescopes are 
highlighted in this chapter including various local setting 
which were executed during the time of observations. 
Details about initial and basic analysis procedures 
followed for all our observations in this thesis work 
are also elaborated. These include, (a) obtaining single pulses 
from different observatories, (b) eliminating radio frequency 
interferences related effects, (c) estimation of the NF 
and (d) obtaining the null and burst length histograms from 
the separated null and burst pulses. A novel approach to isolate 
weak burst pulses among the null pulses is also introduced 
here for the first time. 

% \section*{\underline{\underline{Survey of nulling pulsars using the GMRT}}\\
% (Gajjar, V., Joshi B. C. and Kramer M., 2012, MNRAS, 424, 1197)}
\section*{Survey of nulling pulsars using the GMRT \\
\underline{\underline{(Gajjar, V., Joshi B. C. and Kramer M., 2012, MNRAS, 424, 1197)}}}

In recent years Parkes Multibeam Survey (PKSMB) has discovered many new
pulsars. Several of them show nulling behaviour in their discovery plots. 
We have carefully looked through the discovery plots of many pulsars, out of 
which, 5 promising candidates were selected for longer observations 
with the GMRT. In \emph{Chapter 4}, the nulling behaviour 
of 15 pulsars, which include 5 PKSMB pulsars with no previously 
reported nulling behaviour, with the estimates on 
their NFs is reported. For four of these 15 pulsars, 
only an upper/lower limit was previously reported. 
The estimates of reduction in the pulsed emission is 
also presented for the first time in 11 pulsars. 
NF value for individual profile component is also 
presented for two pulsars in the sample \emph{viz.}  
PSRs B2111+46 and B2020+28. Possible mode changing 
behaviour is suggested by these observations 
for PSR J1725--4043, but this needs to be confirmed with
more sensitive observations. An interesting 
quasi-periodic nulling behaviour for PSR J1738--2330 is also reported. 

We find that the nulling patterns differ between 
PSRs B0809+74, B0818--13, B0835--41 and B2021+51, even though
they have similar NF of around 1\%. We showed this by comparing 
the null length and burst length distributions using a 
two sample Kolmogorov-Smirnov test. Our results 
confirm that NF probably does not capture the full detail 
of the nulling behaviour of a pulsar. Thus, it can be 
speculated that, due to this, earlier attempts failed to correlate 
NF with various pulsar parameters.  

We carried out the Wald-Wolfowitz runs test for randomness 
to 8 more pulsars. We find that this test indicates that 
occurrence of nulling, when individual pulses are considered, is 
non-random or exhibits correlation across periods. 
This correlation groups pulses in null and burst states, 
which was also noted by \cite{rr09}. 
However, the durations of the null and the burst states shown 
to be modelled by a stochastic Poisson point process suggesting that 
these transitions occur at random. 
Thus, the underlying physical process for nulls in the 8 pulsars  
studied appears to be random in nature producing 
nulls and bursts with unpredictable durations. 
Moreover, modelling of the null length and the burst length distributions
provided typical nulling and burst timescale (i.e. $\tau_n$ and $\tau_b$ respectively),  
which were derived for 8 pulsars for the first time to the best of our knowledge. 

\section*{On the long nulls of PSRs J1738$-$2330 and J1752+2359\\
\underline{\underline{(Gajjar, V., Joshi B. C., and Geoffrey W. 2014a, MNRAS,  439, 221)}}}
A detailed study of pulse energy modulation in two pulsars, 
\psra\ and \psrb, with similar NF has been presented in \emph{Chapter 5}. 
The NFs were estimated to be 85$\pm$2\% and 81\% 
for \psra\ and \psrb\ respectively. The aim of this study was to investigate 
similarity and differences between two high NF pulsars. 

Both the pulsars exhibit similar bunching of the burst pulses 
classified as the \emph{bright phases}, which are separated by long 
null phases. A similar quasi-periodic switching between 
these two state is observed for both the pulsars. 
However, using a new technique of pair-correlation-function (PCF), 
we have reported significant differences between these two pulsars. 
The PCF for \psra\ indicates that the mechanism responsible 
for bright phases is governed by two quasi-periodic 
processes with periodicities of 170 and 270 pulses, 
On the other hand, the nulling pattern of \psrb\ is dominated 
by 540 pulse quasi-periodicity, which jitters from 490 to 
595 pulses. These processes are not strictly periodic, 
but retain a memory longer than 2000 pulses for \psra, while 
the memory of \psrb's periodic  structure is retained for only 
about 1000 periods. 

Towards the end of each bright phase of \psrb, an exponential 
decline in the pulse energy is reported. 
\psra\ also shows similar exponential decay 
along with a flickering emission characterized by short frequent 
nulls towards the end of each bright phase. 
We modelled the bright pulse energy decay for 
\psrb\ and estimated their average 
lengths. A strong anti-correlation 
was found between the peak energy and 
the decay time for all bright phases in this pulsar. 
We demonstrated that the area under each bright phase is similar, 
suggesting that the energy release during all such events is 
approximately constant for \psrb.  
The first bright phase pulse profile and the last bright phase 
pulse profile show striking differences between both the pulsars, 
hinting differences in transition from null phase to burst phase and 
vice-versa between the two pulsars. We report, for the first time, 
peculiar weak burst pulses during the long null phases of \psrb, 
which we call as inter-burst pulses (IBPs). 
The IBPs are similar to emission seen from RRATs. 
The occurrence rate of the IBPs is random and uncorrelated with 
the preceding or following bright phase parameters. 
The polarization profiles for \psrb\ obtained from observations 
with the Arecibo telescope are reported for the first time.  
The total intensity and the circular polarization profiles 
of IBPs are slightly shifted towards the leading side 
compared to the conventional integrated profile, 
indicating a change in the emission region. 
No such pulses were seen in the long null phases of 
\psra. Lastly, we do not observe any GPs in 
our long observations unlike such pulses being 
reported at low frequencies in \psrb\ \cite[]{EK05}.
Hence, these results confirm that even though these 
two pulsar have similar but significantly high 
NFs, they show very different nulling behaviour. 


\section*{Simultaneous multi-frequency study of pulse nulling behaviour in two pulsars \\
\underline{\underline{(Gajjar, V., Joshi B. C., Kramer M., Smith R. and Karuppusamy R., 2014b, ApJ, 797, 18)}}}
A detailed study on the simultaneous occurrence of the nulling phenomena
in two pulsars, PSRs B0809+74 and B2319+60, is reported in \emph{Chapter 6}. 
The observations were conducted simultaneously at four different 
frequencies, 313, 607, 1380 and 4850 MHz, from three different 
telescopes \emph{viz.} the GMRT, the WSRT and the Effelsberg radio telescope. 
The overlap time for each pulsar was around 6 hours 
between different observatories. 

We obtained single pulses at each frequency and the on-pulse 
energies were compared across all four frequencies, which showed 
remarkable similarity in the pulse energy fluctuations 
for both the pulsars. To quantify these similarities, we obtained the NF 
at each frequency which were found to be consistence within the error bars, 
at all four frequencies for both the pulsars. 
Similarly, the one-bit sequences were also compared 
using the contingency table analysis. To measure 
the statistical significance of the contingency tables, 
we measured the Cramer-V and the uncertainty coefficient 
for each pair of frequencies. For PSR B0809+74, 
both the statistical tests showed highly 
significant broadband nulling behaviour. For PSR B2319+60, 
the significance was marginally lower for the pairs 
involving 4850 MHz. 

We also scrutinize all the nonconcurrent 
pulses (i.e. pulses which did not show similar emission states 
across different frequencies) for both the pulsars to investigate their true nature. 
For PSR B0809+74, we found that out of 12 nonconcurrent 
pulses, 7 (about 58\%) occurred at the transition point where emission 
state is switching from null to burst (or vice-verse). 
Similarly for PSR B2319+60, we found that out of 158 
nonconcurrent pulses, 82 (about 52\%) occurred at the transition point where 
emission state is switching. Thus, both pulsars showed remarkable 
similarity in the overall broadband behaviour, also accounting the 
fraction of nonconcurrent pulses at the transition points. 

A slight difference can be seen for the \emph{exclusive} 
pulse profiles, pulses which exclusively occurred at a single 
observing frequency, between both the pulsars. PSR B0809+74 
showed significantly narrow pulses (except at 4850 MHz) 
aligning the overall pulse profile, while PSR B2319+60 showed significantly 
weak pulses which are shifted towards the leading edge compared to the overall 
pulse profile. However, a strong claim can not be made regarding 
their true shapes, due to their small numbers. 
We also compared the null length and the burst length distributions across all 
observed frequencies which showed similar distribution with high 
significance ($>$99\%) for both the pulsars. These results clearly suggest 
that nulling is truly a broadband phenomena. It favours models invoking 
magnetospheric changes on a global scale compared to 
local geometric effects as a likely cause of nulling in these pulsars. 

\section*{\underline{\underline{Conclusions}}} 
Final summary of all obtained results are listed in \emph{Chapter 7} and their 
implications are discussed. We have also combined the obtained results 
on three different aspects of the nulling behaviour. 
In light of these results, following interpretations 
about the nulling phenomena can be suggested. 
\begin{enumerate}
 \item NF is not an ideal parameter to quantify nulling behaviour, confirmed firmly 
  by comparing low NF pulsars as well as high NF pulsars.  
 \item Nulling occurs randomly with unpredictable length durations. 
  Quasi-periodicities seen in the high NF pulsars can also be explained 
  by the Markov models with a forcing function.  
 \item Nulling is an extreme form of mode-changing phenomena which 
  occurs on a global magnetospheric scale. 
 \item Geometric reasons are less favoured as a likely cause of nulling phenomena 
  due to the randomness and broadband behaviour reported in this thesis.  
\end{enumerate}
These results can also be extended to 
explain the peculiar emission behaviour seen in the 
intermittent pulsars and the RRATs. 
Future work motivated by these observations are listed 
towards the end of this chapter. 


\section*{List of publications}
\subsection*{Refereed Journal}
\begin{itemize}
 \item Gajjar, V., Joshi B. C. and Kramer M., 2012, \newline
       \emph{Survey of nulling pulsars using the Giant Meterwave Radio Telescope}, \newline
       MNRAS, 424, 1197
       
 \item Gajjar, V., Joshi B. C., and Geoffrey W. 2014a, \newline
       \emph{On the long nulls of PSRs 11738-2330 and J1752+2359}, \newline
       MNRAS, 439, 221

 \item Gajjar, V., Joshi B. C., Kramer M., Smith R. and Karuppusamy R., 2014b, \newline
       \emph{Frequency independent quenching of pulsed emission}, \newline
       ApJ, 797, 18       
\end{itemize}

\subsection*{Proceedings}
\begin{itemize}
 \item Gajjar, V., Joshi B. C. and Kramer M., 2009, \newline
       \emph{Peculiar nulling in PSR J1738-2330}, \newline
       ASP conference series, 407, 304
       
 \item Gajjar, V., Joshi B. C. and Kramer M., 2012, \newline
       \emph{Broadband nulling behaviour of PSR B2319+60}, \newline
       ASP conference proceeding, 466, 79
       
 \item Gajjar, V., Joshi B. C. and Kramer M., 2013, \newline
       \emph{A survey of nulling pulsars using the Giant Meterwave Radio Telescope}, \newline
       Proceedings of IAU Symposium, 291, 385
       
 \item Gajjar, V., Joshi B. C. and Kramer M., 2011, \newline
       \emph{A survey of nulling pulsars using GMRT}, \newline
       Astronomical Society of of India Conference Series, 3, 118
\end{itemize}

% \singlespace
% \bibliographystyle{mn2e.bst}
% \bibliography{/home/vishal/My_paper/Bibfiles/psrrefs.bib,/home/vishal/My_paper/Bibfiles/modpsrrefs.bib,/home/vishal/My_paper/Bibfiles/mybib.bib,/home/vishal/My_paper/Bibfiles/modrefs.bib}

